Embodied Neuromorphic Vision with Event-Driven Random Backpropagation

Spike-based communication between biological neurons is sparse and unreliable. This enables the brain to process visual information from the eyes efficiently. Taking inspiration from biology, artificial spiking neural networks coupled with silicon retinas attempt to model these computations. Recent findings in machine learning allowed the derivation of a family of powerful synaptic plasticity rules approximating backpropagation for spiking networks. Are these rules capable of processing real-world visual sensory data? In this paper, we evaluate the performance of Event-Driven Random Back-Propagation (eRBP) at learning representations from event streams provided by a Dynamic Vision Sensor (DVS). First, we show that eRBP matches state-of-the-art performance on the DvsGesture dataset with the addition of a simple covert attention mechanism. By remapping visual receptive fields relatively to the center of the motion, this attention mechanism provides translation invariance at low computational cost compared to convolutions. Second, we successfully integrate eRBP in a real robotic setup, where a robotic arm grasps objects according to detected visual affordances. In this setup, visual information is actively sensed by a DVS mounted on a robotic head performing microsaccadic eye movements. We show that our method classifies affordances within 100ms after microsaccade onset, which is comparable to human performance reported in behavioral study. Our results suggest that advances in neuromorphic technology and plasticity rules enable the development of autonomous robots operating at high speed and low energy consumption.

==> extra.tex <==
\subsection{N-MNIST}
The N-MNIST dataset was recorded using a \ac{DVS} in front of an LCD screen displaying moving MNIST digits.
This motion pattern is the same for all samples and represents saccadian movements of our eyes.
The schematic digit motion can be seen in \cref{fig:exp66:sacc_mov_hist} and \cref{fig:exp66:sacc_mov_arrows}.
This data set consists only of a subset of the original MNIST data set.
With only 9000 training samples and 1000 test samples this data set is significantly smaller than the original MNIST.
These samples were downsampled from $128\times 128$ to $32\times 32$.
Specifically, one neuron in the input layer is spiking for each event within a $4\times 4$ neighbourhood of event coordinates.

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{0.45\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{img/saccadian_mnist/saccade.png}
        \caption{}
        \label{fig:exp66:sacc_mov_hist}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{img/saccadian_mnist/saccade_arrows.pdf}
        \caption{}
        \label{fig:exp66:sacc_mov_arrows}
    \end{subfigure}
    \caption{S-MNIST: Saccadian movement.
      These two images demonstrate the saccadian digit motion.
      (\subref{fig:exp66:sacc_mov_hist}): The image shows an event histogram of a sample of label one.
      The digit border indicates the amplitude of the movement.
      (\subref{fig:exp66:sacc_mov_arrows}): The arrows show the 45\degree\ motion directions and their order.
      The complete motion in the arrow directions 1 to 4 is executed twice for each sample.
    }
\end{figure}


The network reaches an accuracy of X\% on N-MNIST after X epochs, see \cref{fig:exp66:acc_rate_first}.
The microsaccadic eye movements are clearly visible in the spiking activity of the network depicted in \cref{fig:exp66:spiketrains}.
Over time, the number of synaptic weight updates remained low, important for a neuromorphic hardware implementation.

\begin{figure}[!htbp]
\centering
\includegraphics[width=\columnwidth]{saccadian_mnist/exp66/acc_rate_first.png}
\caption{
S-MNIST: Classification accuracy over epochs.
The classification accuracy over all 30 epochs using the output spiking rate is represented by the blue curve, which has its maximum at 83.5\%.
Classification using the first output spike, shown in red, was working less reliable with a maximum of 62\% accuracy.
}
\label{fig:exp66:acc_rate_first}
\end{figure}

\begin{figure}[!htbp]
\centering
\includegraphics[width=\columnwidth,clip=true,trim=0 0 0 2.7cm]{img/saccadian_mnist/exp66/spiketrains.png}
\caption{
S-MNIST: Network spiking behaviour.
This is the spiking behaviour of input, hidden and output layers.
The top most graph shows spikes at the label neurons 8, 2 and 7 for these three samples.
In the input graph the 4 different motion directions repeated twice can be seen for each sample.
The first hidden layer consists of hidden neurons 0-199 and the second hidden layer is using hidden neurons 200-399.
At the output the correct neurons spike the most over the time of the samples, which is why these samples were correctly classified.
}
\label{fig:exp66:spiketrains}
\end{figure}

%% As mentioned in \cite{iyer2018neuromorphic}, N-MNIST does not carry information in the time domain and is therefore a bad benchmark for spiking networks.
%% In the next section, we benchmark \cite{eRBP} on DvsGesture which does carry temporal information.

